Regular Potential Games

A fundamental problem with the Nash equilibrium concept is the existence of certain "structurally deficient" equilibria that (i) lack fundamental robustness properties, and (ii) are difficult to analyze. The notion of a "regular" Nash equilibrium was introduced by Harsanyi. Such equilibria are isolated, highly robust, and relatively simple to analyze. A game is said to be regular if all equilibria in the game are regular. In this paper it is shown that almost all potential games are regular. That is, except for a closed subset with Lebesgue measure zero, all potential games are regular. As an immediate consequence of this, the paper also proves an oddness result for potential games: in almost all potential games, the number of Nash equilibrium strategies is finite and odd. Specialized results are given for weighted potential games, exact potential games, and games with identical payoffs. Applications of the results to game-theoretic learning are discussed.

==> authors_and_title.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\usepackage{hyperref}

\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Declare title and authors, without \thanks
\newcommand{\TheTitle}{Regular Potential Games}
\newcommand{\TheAuthors}{B. Swenson, R. Murray, and S. Kar}

% Sets running headers as well as PDF title and authors
%\headers{\TheTitle}{\TheAuthors}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{{\TheTitle}}

%% Authors: full names plus addresses.
%\author{
%  Brian Swenson\thanks{Department of Electrical and Computer Engineering, Carnegie Mellon University, Pittsburgh, PA and Institute for Systems and Robotics (ISR/IST), LARSyS, Instituto Superior T\'{e}cnico, University of Lisbon (\email{brianswe@ece.cmu.edu}).}
%  \and
%  Ryan Murray\thanks{Department of Mathematics, Pennsylvania State University, State College, PA (\email{rwm22@psu.edu}).}
%  \and
%  Soummya Kar\thanks{Department of Electrical and Computer Engineering, Carnegie Mellon University, Pittsburgh, PA    (\email{soummyak@andrew.cmu.edu}).}
%}



\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables:
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End:

